ReRoGCRL: Representation-based Robustness in Goal-Conditioned Reinforcement Learning

While Goal-Conditioned Reinforcement Learning (GCRL) has gained attention, its algorithmic robustness against adversarial perturbations remains unexplored. The attacks and robust representation training methods that are designed for traditional RL become less effective when applied to GCRL. To address this challenge, we first propose the Semi-Contrastive Representation attack, a novel approach inspired by the adversarial contrastive attack. Unlike existing attacks in RL, it only necessitates information from the policy function and can be seamlessly implemented during deployment. Then, to mitigate the vulnerability of existing GCRL algorithms, we introduce Adversarial Representation Tactics, which combines Semi-Contrastive Adversarial Augmentation with Sensitivity-Aware Regularizer to improve the adversarial robustness of the underlying RL agent against various types of perturbations. Extensive experiments validate the superior performance of our attack and defence methods across multiple state-of-the-art GCRL algorithms. Our tool ReRoGCRL is available at https://github.com/TrustAI/ReRoGCRL.

==> Tables/layer_ablation.tex <==
\begin{tabular}{@{}cc|c|c|c|c@{}}
\toprule
\multicolumn{2}{c|}{Methods}                                                                                      & FetchPick             & FetchPush             & FetchReach            & FetchSlide \\ \midrule
\multirow{3}{*}{DDPG}  & \multicolumn{1}{c|}{layer -1}                           &9.91\scriptsize{$\pm$3.93}  &6.89\scriptsize{$\pm$2.39}  &2.46\scriptsize{$\pm$6.14}  &0.11\scriptsize{$\pm$0.52}            \\
 
& \multicolumn{1}{c|}{layer -2}  &9.56\scriptsize{$\pm$5.13}
&7.24\scriptsize{$\pm$3.25} 
&2.46\scriptsize{$\pm$1.87}  &0.00\scriptsize{$\pm$0.00}            \\
& \multicolumn{1}{c|}{layer -3}                &7.83\scriptsize{$\pm$}3.06 
&6.43\scriptsize{$\pm$}2.33 
&2.02\scriptsize{$\pm$}3.32
&0.00\scriptsize{$\pm$}0.00
%                        \\ \midrule
% \multirow{3}{*}{GCSL} & \multicolumn{1}{c|}{layer -1}                     &8.29\scriptsize{$\pm$}1.83
% &11.53\scriptsize{$\pm$}3.99
% &22.21\scriptsize{$\pm$6.76} 
% &0.75\scriptsize{$\pm$0.00}
% \\
% & \multicolumn{1}{c|}{layer -2} &8.79\scriptsize{$\pm$4.40} &6.93\scriptsize{$\pm$}3.76
% &23.17\scriptsize{$\pm$6.46} &0.86\scriptsize{$\pm$0.00}            \\
% & \multicolumn{1}{c|}{layer -3}                &8.99\scriptsize{$\pm$}3.26 &8.99\scriptsize{$\pm$}3.99  &23.04\scriptsize{$\pm$}4.48 &0.37\scriptsize{$\pm$}0.00         
\\ \bottomrule
\end{tabular}

==> Tables/table_DisReturn_layer-3_epsilon_0.1_ddpg.tex <==
{\scriptsize
\begin{tabular}{@{}c|ccccccc@{}}
\toprule
&   \multicolumn{7}{c}{DDPG}         \\     
\multirow{-2}{*}{Task}         
 & Clean   & Uniform & Gaussian & SA-FGSM & SA-PGD  & \textbf{C-FGSM} & \textbf{C-PGD-20} \\ \midrule
\multicolumn{1}{l|}{FetchReach}  &29.92      &28.86  &28.86      &24.21       &20.14       &0.70   &0.78 \\
\multicolumn{1}{l|}{FetchPick}  &14.82 &16.68 &16.68 &19.61 &19.92 &11.18 &10.97     \\
\multicolumn{1}{l|}{FetchPush}  &12.81 &13.61 &13.61 &17.24 &15.42 &6.22 &6.98 \\
\multicolumn{1}{l|}{FetchSlide} &0.58 &1.89 &1.89 &0.59 &0.50 &0.00 &0.09 \\ 
\bottomrule              
\end{tabular}
}

==> Tables/table_DisReturn_layer-3_epsilon_0.1_gofar.tex <==
{\scriptsize
\begin{tabular}{@{}c|ccccccc@{}}
\toprule
&   \multicolumn{7}{c}{GoFar}         \\     
\multirow{-2}{*}{Task}         
 & Clean   & Uniform & Gaussian & SA-FGSM & SA-PGD  & \textbf{C-FGSM} & \textbf{C-PGD-20} \\ \midrule

\multicolumn{1}{l|}{FetchPick}  &     \\
\multicolumn{1}{l|}{FetchPush}  &18.38 &1.90 &1.90 &1.90 &1.90 &1.90 &1.90 \\
\multicolumn{1}{l|}{FetchReach}  &      &         &         &       &       &   & \\
\multicolumn{1}{l|}{FetchSlide} & \\ 
\bottomrule              
\end{tabular}
}

==> Tables/table_DisReturn_layer-3_epsilon_0.1_simsr+ddpg.tex <==
\begin{tabular}{@{}c|ccccccc@{}}
\toprule
&   \multicolumn{7}{c}{SimSR + DDPG}         \\     
\multirow{-2}{*}{Task}         
 & Clean   & Uniform & Gaussian & SA-FGSM & SA-PGD  & \textbf{SCR-FGSM} & \textbf{SCR-PGD} \\ \midrule
\multicolumn{1}{l|}{FetchPick}  &16.78 &16.00 &16.00 &19.51 &17.92 &15.74 &16.15 \\
\multicolumn{1}{l|}{FetchPush}  &12.63 &15.43 &15.43 &16.24 &14.61 &10.70 &10.51\\
\multicolumn{1}{l|}{FetchReach}  &29.90 &29.46 &29.46 &28.68 &26.76 &27.72 &27.16 \\
\multicolumn{1}{l|}{FetchSlide} &0.62 &0.83 &0.83 &0.80 &0.43 &0.37 &0.84 \\ 
\bottomrule              
\end{tabular}


==> Tables/table_DisReturn_layer-3_epsilon_0.1_simsr+gofar.tex <==
\begin{tabular}{@{}c|ccccccc@{}}
\toprule
&   \multicolumn{7}{c}{SimSR + GoFar}         \\     
\multirow{-2}{*}{Task}         
 & Clean   & Uniform & Gaussian & SA-FGSM & SA-PGD  & \textbf{SCR-FGSM} & \textbf{SCR-PGD} \\ \midrule
\multicolumn{1}{l|}{FetchPick}  &17.44 &16.73 &16.73 &17.63 &13.80 &16.27 &16.11 \\
\multicolumn{1}{l|}{FetchPush}  &14.19 &13.13 &13.13 &15.52 &13.91 &12.44 &13.08\\
\multicolumn{1}{l|}{FetchReach}  &27.93 &27.91 &27.91 &27.95 &27.96 &27.96 &27.98 \\
\multicolumn{1}{l|}{FetchSlide} &1.66 &1.78 &1.78 &2.31 &1.41 &1.07 &0.59 \\ 
\bottomrule              
\end{tabular}


==> Tables/table_SuccRate_layer-1_epsilon_0.075_ddpg.tex <==
\begin{tabular}{@{}c|ccccccc@{}}
\toprule
& \multicolumn{7}{c}{DDPG} \\
Task           &   Clean   & Uniform & Gaussian & SA-FGSM & SA-PGD  & \textbf{Contrastive-FGSM} & \textbf{Contrastive-PGD-20}                  \\ \midrule
FetchReach & 1.00     &  0.98       &  0.98      & 0.78     &  \textbf{0.61}   & 0.86               &   0.82                 \\
FetchPick  &  0.68  &    0.76   &  0.76     &  0.86    &  0.86    &   0.64            &    \textbf{0.60}                \\
FetchPush  & 0.68 & 0.80    & 0.80     & 0.86 & 0.86 & \textbf{0.42}             & 0.64               \\
FetchSlide & 0.04  &  0.20  &  0.20    &  0.04  & \textbf{0.00}   &  \textbf{0.00}          &   0.02  \\ 
\bottomrule              
\end{tabular}

==> Tables/table_SuccRate_layer-1_epsilon_0.1_ddpg.tex <==
{\scriptsize
\begin{tabular}{@{}c|ccccccc|ccccccc@{}}
\toprule
&   \multicolumn{7}{c|}{DDPG}                                                        & \multicolumn{7}{c}{GCSL}        \\     
\multirow{-2}{*}{Task}         
 & Clean   & Uniform & Gaussian & SA-FGSM & SA-PGD  & \textbf{C-FGSM} & \textbf{C-PGD-20} & Clean & Uniform & Gaussian & SA-FGSM & SA-PGD & \textbf{C-FGSM} & \textbf{C-PGD} \\ \midrule
\multicolumn{1}{l|}{FetchReach}  &  1.00    & 0.98        &   0.98       &   0.72    & \textbf{0.58}      &  0.86                &    0.80 &1.00 &1.00 &1.00 &1.00 &1.00 &1.00 &1.00   \\
\multicolumn{1}{l|}{FetchPick}  & 0.68 & 0.76    & 0.76     & 0.86 & 0.86 & \textbf{0.64}             & 0.68    &0.62 &0.64 &0.64 &0.56 &0.54 &\textbf{0.38} & \textbf{0.38}                \\
\multicolumn{1}{l|}{FetchPush}  & 0.68 & 0.82    & 0.82     & 0.86 & 0.76 & \textbf{0.54}         & 0.56  &0.72 &0.76 &0.76 &0.64 &0.64 &0.46 &\textbf{0.34}              \\
\multicolumn{1}{l|}{FetchSlide} &0.04 &0.2     &0.2 &0.04 &0.04 & \textbf{0.02}    &\textbf{0.02} &0.16 &0.18 &0.18 &0.06 &0.04 &\textbf{0.00} &\textbf{0.00}   \\ 
\bottomrule              
\end{tabular}
}

==> Tables/table_SuccRate_layer-3_epsilon_0.1_ddpg.tex <==
{\scriptsize
\begin{tabular}{@{}c|ccccccc|ccccccc@{}}
\toprule
&   \multicolumn{7}{c|}{DDPG}                                                        & \multicolumn{7}{c}{GCSL}        \\     
\multirow{-2}{*}{Task}         
 & Clean   & Uniform & Gaussian & SA-FGSM & SA-PGD  & \textbf{C-FGSM} & \textbf{C-PGD-20} & Clean & Uniform & Gaussian & SA-FGSM & SA-PGD & \textbf{C-FGSM} & \textbf{C-PGD} \\ \midrule
\multicolumn{1}{l|}{FetchReach}  &  1.00    & 0.98        &   0.98       &   0.72    & \textbf{0.58}      &  0.70                &    0.78 &1.00 &1.00 &1.00 &1.00 &1.00 &1.00 &1.00   \\
\multicolumn{1}{l|}{FetchPick}  & 0.68 & 0.74    & 0.74     & 0.84 & 0.90 & 0.60             & \textbf{0.54}    &0.62 &0.64 &0.64 &0.56 &0.54 & 0.52 & \textbf{0.50}                \\
\multicolumn{1}{l|}{FetchPush}  & 0.68 & 0.82    & 0.82     & 0.86 & 0.76 & \textbf{0.34}         & \textbf{0.34}  &0.72 &0.76 &0.76 &0.64 &0.64 &\textbf{0.40} &\textbf{0.40}              \\
\multicolumn{1}{l|}{FetchSlide} &0.04 &0.2     &0.2 &0.04 &0.04 & \textbf{0.02}    &\textbf{0.02} &0.16 &0.18 &0.18 &0.06 &0.04 &\textbf{0.04} &\textbf{0.04}   \\ 
\bottomrule              
\end{tabular}
}

==> Tables/table_sgld_attack.tex <==
{
\begin{tabular}{@{}c|cccccccccc@{}}
\toprule
&   \multicolumn{10}{c}{\textbf{DDPG+SGLD} (3 seeds)}         \\     
\multirow{-1}{*}{Task}         
 & Nature & Uniform& SA-FGSM & SA-PGD  & \multicolumn{3}{c}{SCR-FGSM} & \multicolumn{3}{c}{SCR-PGD}
 \\
 & & & & &  state & goal & state+goal & state & goal & state+goal
  
\\ \midrule
\multicolumn{1}{l|}{FetchPick}  
&15.46\scriptsize{$\pm$}1.50
&16.20\scriptsize{$\pm$}2.64 
&18.58\scriptsize{$\pm$}3.18 
&18.09\scriptsize{$\pm$}2.44 
&10.94\scriptsize{$\pm$}2.09 
&15.51\scriptsize{$\pm$}2.28 
&\textbf{7.62}\scriptsize{$\pm$}4.27 
&8.84\scriptsize{$\pm$}3.29 
&17.38\scriptsize{$\pm$}1.81 
&11.41\scriptsize{$\pm$}3.20  \\
\multicolumn{1}{l|}{FetchPush}  &11.04\scriptsize{$\pm$}5.52
&10.56\scriptsize{$\pm$}4.22 
&13.72\scriptsize{$\pm$}0.87 
&12.74\scriptsize{$\pm$}5.17 &6.76\scriptsize{$\pm$}2.42 &9.40\scriptsize{$\pm$}4.74 &5.80\scriptsize{$\pm$}2.57  &8.30\scriptsize{$\pm$}0.98 &12.22\scriptsize{$\pm$}2.41 &\textbf{3.72}\scriptsize{$\pm$}1.94\\
\multicolumn{1}{l|}{FetchReach}  &29.81\scriptsize{$\pm$}0.16 &28.66\scriptsize{$\pm$}0.50 &25.01\scriptsize{$\pm$}2.53
&23.62\scriptsize{$\pm$}2.58 &9.34\scriptsize{$\pm$}8.16 &8.09\scriptsize{$\pm$}8.38 &3.37\scriptsize{$\pm$}3.90 &25.82\scriptsize{$\pm$}2.05 &14.65\scriptsize{$\pm$}8.60 &\textbf{3.10}\scriptsize{$\pm$}4.02 \\
\multicolumn{1}{l|}{FetchSlide} &0.97\scriptsize{$\pm$}1.68 
&0.97\scriptsize{$\pm$}1.12 
&0.84\scriptsize{$\pm$}1.45 
&0.11\scriptsize{$\pm$}0.20 
&0.01\scriptsize{$\pm$}0.02 
&0.60\scriptsize{$\pm$}0.91 
&0.00\scriptsize{$\pm$}0.00
&0.00\scriptsize{$\pm$}0.00 
&0.03\scriptsize{$\pm$}0.06 
&0.00\scriptsize{$\pm$}0.00
\\ 
\bottomrule              
\end{tabular}

% \begin{tabular}{@{}c|cccccc@{}}
% \toprule
% &   \multicolumn{6}{c}{GoFar (SimSR)}         \\           
%  & Nature & Uniform& SA-FGSM & SA-PGD  & SCR-FGSM & SCR-PGD \\ \midrule
%  &17.44 &16.73 &17.63 & \textbf{13.80} &16.27 &16.11 \\
% &14.19 &13.13 &15.52 &13.91 & \textbf{12.44} &13.08\\
%  &27.93 & \textbf{27.91} &27.95 &27.96 &27.96 &27.98 \\
% &1.66 &1.78 &2.31 &1.41 &1.07 & \textbf{0.59} \\ 
% \bottomrule              
% \end{tabular}
}

==> Tables/table_sgld_defence.tex <==
\begin{tabular}{@{}cc|c|c|c|c@{}}
\toprule
\multicolumn{2}{c|}{Methods}                                                                                      & FetchPick             & FetchPush             & FetchReach            & FetchSlide \\ \midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}
{DDPG}}  
& \multicolumn{1}{c|}{Vanilla}                           &7.83\scriptsize{$\pm$3.06}  &5.42\scriptsize{$\pm$3.00}  &1.86\scriptsize{$\pm$3.31}  &0.00\scriptsize{$\pm$0.00}            \\
 
& \multicolumn{1}{c|}{Vanilla+SCAA}  &\textbf{14.53\scriptsize{$\pm$3.08}}
&\textbf{10.79\scriptsize{$\pm$4.55}} 
&\textbf{27.68\scriptsize{$\pm$1.30}}  &\textbf{0.00\scriptsize{$\pm$0.00}}            \\
& \multicolumn{1}{c|}{\textcolor{purple}{Vanilla+SGLD}}            
&\textcolor{purple}{7.62\scriptsize{$\pm$}4.27 }
&\textcolor{purple}{3.72\scriptsize{$\pm$}1.94}  &\textcolor{purple}{3.10\scriptsize{$\pm$}4.02} &\textcolor{purple}{0.00\scriptsize{$\pm$}0.00} \\ 

& \multicolumn{1}{c|}{SimSR}                &15.74\scriptsize{$\pm$}0.65 
&10.51\scriptsize{$\pm$}5.79 
&27.16\scriptsize{$\pm$}2.75
&0.37\scriptsize{$\pm$}0.60 \\
& \multicolumn{1}{c|}{SimSR+SAR}
&\textbf{16.78\scriptsize{$\pm$}1.39}       &\textbf{12.63\scriptsize{$\pm$3.89}} 
&\textbf{29.91\scriptsize{$\pm$0.20}}
&\textbf{0.55\scriptsize{$\pm$0.20}} \\         
\bottomrule
\end{tabular}
